Price of Safety in Linear Best Arm Identification

We introduce the safe best-arm identification framework with linear feedback, where the agent is subject to some stage-wise safety constraint that linearly depends on an unknown parameter vector. The agent must take actions in a conservative way so as to ensure that the safety constraint is not violated with high probability at each round. Ways of leveraging the linear structure for ensuring safety has been studied for regret minimization, but not for best-arm identification to the best our knowledge. We propose a gap-based algorithm that achieves meaningful sample complexity while ensuring the stage-wise safety. We show that we pay an extra term in the sample complexity due to the forced exploration phase incurred by the additional safety constraint. Experimental illustrations are provided to justify the design of our algorithm.

==> apps/algorithms.tex <==
\section{Alternative algorithms}
\label{section:safe_lingape_alternate}

In this section, we provide pseudo-code for the alternative algorithms presented in the experiments.

\begin{remark}
In all experiments, $\gamma$ parameters are updated at each time step given our current estimate of the safe set. If criterion \ref{crit:prob_safe} is chosen in order to select the arms, the optimization problem \eqref{opt:simple-weights} is solved every $T_\mathrm{opt}$ time steps. For the sake of lightness, this step is not written in the pseudo code.
\end{remark}

\subsection{Optimistic \SafeLGapE}

\SafeLGapEO is very similar to \SafeLGapE, the main difference between the two algorithms being the the input of the select-direction function (Algorithm~\ref{alg:safe-bai-conservative}). Within this function, instead of considering a conservative pessimistic estimate of the safe set, \SafeLGapEO look at upper confidence bounds on the safety signal in order to define an alternative safe set $\mathcal{S}^\mathrm{opt}_t$. However, in order to ensure safety, when pulling an arm, the pessimistic safe set is considered.

The pseudo code of \SafeLGapE is displayed in Algorithm~\ref{alg:safe-bai-optimistic}. Note that the select-direction(t, $\mathcal{S}^\mathrm{opt}_t$) on Line 12 corresponds to the select-direction of Algorithm~\ref{alg:safe-bai-conservative} where the set $\mathcal{S}^\mathrm{opt}_t$ is considered instead of $\mathcal{S}^\mathrm{pes}_t$.

\begin{algorithm}[t!]
  \caption{\SafeLGapEO}
  \label{alg:safe-bai-optimistic}
  \begin{algorithmic}[1]
    \STATE \textbf{Input}: accuracy $\varepsilon$, safety confidence level $\delta'_\mathrm{s}$, BAI confidence level $\delta_\mathrm{r}$, noise level $R$, norm $D$, regularization parameter $\lambda$, safety bound $\overline{\gamma}$
    \STATE \textbf{Initialization}: $\bA_0 \leftarrow \lambda \bI_d, \bb^{(\mathrm{r})}_0 \leftarrow \mathbf{0}, \bb^{(\mathrm{s})}_0 \leftarrow \mathbf{0}, \safeset' \leftarrow \overline{\gamma} \cX$
    \STATE \textcolor{blue}{$\#$ forced-exploration phase}
    \FOR{$t=1,\dots,T_\mathrm{FE}$}
    \STATE Uniformly sample arms $\hat\bx_t \in \mathcal{S'}$ 
    \STATE Observe reward $r_t = \hat{\bx}_t^\top\btheta^\star + \epsilon_t$
    \STATE Observe safety $s_t = \hat{\bx}_t^\top\bmu^\star + \epsilon'_t$
    \STATE Update $\bA_t$ and $\bb_t$ following~\eqref{eq:update_mean}
    \ENDFOR
    
    %Construct a confidence set $\mathcal{C}_t$ that contains $\btheta^*$ with high probability.
    \STATE \textcolor{blue}{$\#$ loop phase}
    \FOR{$t=T_\mathrm{FE}+1,\dots$}
    \STATE Compute pessimistic safe set $\mathcal{S}^\mathrm{pes}_t$ and optimistic safe set $\mathcal{S}^\mathrm{opt}_t$
    %\STATE Identify the optimistically best arm $x_i$ in $\mathcal{S}_t$\label{safe_lingape:best-arm}
    %\STATE Identify the arm with the smallest optimistic gap with the best arm in $\mathcal{S}_t$
    \STATE $\bx_\mathrm{max}(t), \bx_\mathrm{opt}(t), B(t) \gets$ select-direction$(t, \mathcal{S}^\mathrm{opt}_t)$
    \STATE \textcolor{blue}{$\#$ stopping criterion}
    \IF{$B(t)\leq\varepsilon$}
    \STATE \textbf{return} $\bx_\mathrm{max}(t)$ as the decision
    \ENDIF
    \STATE \textcolor{blue}{$\#$ select which arm to pull}
    \STATE Pull the arm $\bx_\mathrm{pul}(t) \in \mathcal{S}^\mathrm{pes}_t$ according to \eqref{crit:greedy_safe} or \eqref{crit:prob_safe}
    \STATE Observe reward $r_t = \bx_\mathrm{pul}(t)^\top\btheta^\star + \epsilon_t$
    \STATE Update $\bA_t$ and $\bb_t$ following~\eqref{eq:update_mean}
    \ENDFOR
  \end{algorithmic}
\end{algorithm}

\subsection{\SafeLGapE with fixed \texorpdfstring{$\gamma$}{}}

\SafeLGapEF is a simplified version of \SafeLGapE in which $\gamma$ parameters are first estimated in the forced-exploration phase. Those parameters are then fixed and $\LGapE$ is run on the updated bandit model. When $\LGapE$ returns the best arm, $\gamma$ parameters are updated and $\LGapE$ is rerun on the new bandit model. This process terminates when there is no need to sample the new bandit model in order to find the best arm. In Algorithm~\ref{alg:safe-bai-fixed}, $T^{\LGapE}$ corresponds to the termination time of the $\LGapE$ algorithm.

\begin{algorithm}[t!]
  \caption{\SafeLGapEF}
  \label{alg:safe-bai-fixed}
  \begin{algorithmic}[1]
    \STATE \textbf{Input}: accuracy $\varepsilon$, safety confidence level $\delta'_\mathrm{S}$, BAI confidence level $\delta_\mathrm{I}$, noise level $R$, norm $D$, regularization parameter $\lambda$, safety bound $\overline{\gamma}$
    \STATE \textbf{Initialization}: $\bA_0 \leftarrow \lambda \bI_d, \bb^{(\mathrm{r})}_0 \leftarrow \mathbf{0}, \bb^{(\mathrm{s})}_0 \leftarrow \mathbf{0}, \safeset' \leftarrow \overline{\gamma} \cX$
    \STATE \textcolor{blue}{$\#$ forced exploration phase}
    \FOR{$t=1,\dots,T_\mathrm{FE}$}
    \STATE Uniformly sample arms $\hat\bx_t \in \mathcal{S'}$ 
    \STATE Observe reward $r_t = \hat{\bx}_t^\top\btheta^\star + \epsilon_t$
    \STATE Observe safety $s_t = \hat{\bx}_t^\top\bmu^\star + \epsilon'_t$
    \STATE Update $\bA_t$ and $\bb_t$ following~\eqref{eq:update_mean}
    \ENDFOR
    \STATE Compute pessimistic safe set $\mathcal{S}_t$
    \STATE \textcolor{blue}{$\#$ loop phase}
    \WHILE{$T^{\LGapE} \neq 0$}
    \STATE Run \LGapE on the bandit defined on $\mathcal{S}_t$
    \STATE Compute pessimistic safe set $\mathcal{S}_{t+1}$
    \STATE $T^{\LGapE} \leftarrow T^{\LGapE}-1$
    \ENDWHILE
  \end{algorithmic}
\end{algorithm}

==> secs/rebuttal.tex <==
\begin{itemize}
    \item Reviewer 1
    \begin{itemize}
        \item "Framework" vs analysis and algorithm:...
        \item Reference
        \item Justification for $\gamma$
        \item $\Bar{\gamma}$: pas sur de voir ce qu'il veut dire
        \item Details on algorithm and analysis
    \end{itemize}
    \item Reviewer 2
    \begin{itemize}
        \item Regret vs BAI...
        \item Inconsistencies in the notations
        \item $\hat{x} \in X$?
        \item Justification of $\gamma$
    \end{itemize}
    \item Reviewer 3
    \begin{itemize}
        \item Pas $(\epsilon, \delta_I)$ PAC?
        \item Setting $T_{FE}$
        \item Societal impact lol
    \end{itemize}
    \item Reviewer 4
    \begin{itemize}
        \item Structure des bras (cf. reviewer 1 et 2)
        \item Setting $T_{FE}$
        \item Weakness of th6: 
    \end{itemize}
\end{itemize}

==> secs/todo.tex <==
% \section{TODO}

% \begin{itemize}
%     \item Section \ref{sec:safe_bandits}: justifier les bras paramétrisés
%     \item Tout réécrire avec les gamma
% \end{itemize}

% \textbf{Outline}
% \begin{enumerate}
%     \item Introduction
%     \item Related Work
%     \item Problem Formulation: \textbf{Xuedong} -> \textbf{6 mai}
%     \begin{enumerate}
%         \item Unsafe BAI (goal, OLS, \emph{etc.})
%         \item Safety set (definition, impact on the arm set structure)
%     \end{enumerate}
%     \item Proposed Approach
%     \begin{enumerate}
%         \item Forced exploration
%         \item LCB LinGapE: Igor -> ?
%         \item Analysis: \textbf{Igor} -> \textbf{6 mai}
%     \end{enumerate}
%     \item Discussion \& Extensions
%     \item Experiments: \textbf{Merwan} -> ?
%     \item Conclusion
% \end{enumerate}
